PAPR-Limited Precoding in Massive MIMO Systems with Reflect- and Transmit-Array Antennas

Conventional hybrid analog-digital architectures for millimeter-wave massive multiple-input multiple-output (MIMO) systems suffer from poor scalability and high implementational costs. The former is caused by the high power loss in the analog network, and the latter is due to the fact that classic MIMO transmission techniques require power amplifiers with high back-offs. This paper proposes a novel hybrid analog-digital architecture which addresses both of these challenges. This architecture implements the analog front-end via a passive reflect- or transmit-array to resolve the scalability issue. To keep the system cost-efficient, a digital precoder is designed whose peak-to-average power ratio (PAPR) on each active antenna is tunable. Using the approximate message passing algorithm, this precoder is implemented with tractable computational complexity. The proposed architecture allows for the use of power amplifiers with low back-offs which reduces the overall radio frequency cost of the system. Numerical results demonstrate that for low PAPRs, significant performance enhancements are achieved compared to the state of the art.

==> Figs/Revise1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44706,0.74118}%
%
\begin{tikzpicture}

\begin{axis}[%
width=11.076in,
height=6.995in,
at={(1.858in,0.944in)},
scale only axis,
xmin=1.5,
xmax=6.5,
ymin=-7,
ymax=2,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
1.82354091089179	1.25757122339784\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
1.98318991889624	0.518290321838211\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
2.12885592096199	-0.124745774610862\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
2.33190636651553	-1.02110396046365\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
2.57652399299829	-1.73540894579278\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
2.80509939456037	-2.56239113006664\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
3.02131714978317	-3.10663535472137\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
3.15266757966406	-3.46299463556856\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
3.35685684376248	-3.84419095865347\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
3.47983949243154	-4.22931290376892\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
3.65525893764437	-4.54384061412294\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
3.8368240849329	-4.93072239640694\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
4.02238399782767	-5.25357546808593\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
4.29349757932355	-5.57078205256302\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
4.63407100519848	-6.04635822798689\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
4.87136774785384	-6.27009441737223\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
5.37865808394189	-6.65238222619958\\
};
\addplot [color=mycolor1, draw=none, mark size=5.0pt, mark=o, mark options={solid, mycolor1}, forget plot]
  table[row sep=crcr]{%
5.81670232922919	-6.73495600255744\\
};
\addplot [color=mycolor1, dashed, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
1.82354091089179	1.19740541200162\\
1.9	0.851972808937781\\
1.9012163615359	0.846559705110513\\
1.91409726027397	0.789393741827734\\
1.92819452054795	0.727158058586834\\
1.94229178082192	0.66526479077023\\
1.95638904109589	0.603712969933062\\
1.97048630136986	0.542501627630477\\
1.98318991889624	0.487632435733564\\
1.98458356164384	0.481629795417614\\
1.99868082191781	0.421096504849626\\
2.01277808219178	0.360900787481645\\
2.02687534246575	0.301041674868827\\
2.04097260273973	0.241518198566308\\
2.0550698630137	0.182329390129237\\
2.06916712328767	0.123474281112756\\
2.08326438356164	0.0649519030720036\\
2.08733530440183	0.0481139454828465\\
2.09736164383562	0.00676128756213146\\
2.11145890410959	-0.0510985338617189\\
2.12555616438356	-0.108628529644404\\
2.12885592096199	-0.122047087562439\\
2.13965342465753	-0.16582966823078\\
2.15375068493151	-0.222702918065703\\
2.16000725848124	-0.247839310714959\\
2.16784794520548	-0.279249247594029\\
2.18194520547945	-0.335469625260611\\
2.19604246575342	-0.39136501951031\\
2.2101397260274	-0.44693639878798\\
2.22423698630137	-0.502184731538474\\
2.23833424657534	-0.55711098620665\\
2.25243150684932	-0.611716131237367\\
2.26652876712329	-0.666001135075479\\
2.28062602739726	-0.719966966165838\\
2.29472328767123	-0.773614592953308\\
2.30882054794521	-0.826944983882738\\
2.32291780821918	-0.879959107398987\\
2.33190636651553	-0.913596786470434\\
2.33701506849315	-0.932657931946913\\
2.35111232876712	-0.985042425971365\\
2.3652095890411	-1.03711355791721\\
2.37930684931507	-1.08887229622929\\
2.39340410958904	-1.14031960935247\\
2.40750136986301	-1.19145646573161\\
2.42159863013699	-1.24228383381156\\
2.43489585030199	-1.28994390447652\\
2.43569589041096	-1.29280268203717\\
2.44979315068493	-1.34301397885331\\
2.4638904109589	-1.39291869270482\\
2.47798767123288	-1.44251779203658\\
2.49208493150685	-1.49181224529341\\
2.50618219178082	-1.5408030209202\\
2.52027945205479	-1.58949108736179\\
2.53437671232877	-1.63787741306304\\
2.54847397260274	-1.6859629664688\\
2.56257123287671	-1.73374871602394\\
2.57652399299829	-1.78075039101609\\
2.57666849315068	-1.7812356301733\\
2.59076575342466	-1.82842467736174\\
2.60486301369863	-1.87531682603412\\
2.6189602739726	-1.9219130446353\\
2.63305753424658	-1.96821430161013\\
2.64715479452055	-2.01422156540347\\
2.66125205479452	-2.05993580446016\\
2.67534931506849	-2.10535798722508\\
2.67562068027904	-2.10622948284475\\
2.68944657534247	-2.15048908214307\\
2.70354383561644	-2.19533005765899\\
2.71764109589041	-2.2398818822177\\
2.73173835616438	-2.28414552426405\\
2.74583561643836	-2.3281219522429\\
2.75993287671233	-2.37181213459911\\
2.7740301369863	-2.41521703977752\\
2.78812739726027	-2.458337636223\\
2.80222465753425	-2.50117489238041\\
2.80509939456037	-2.50987564420752\\
2.81632191780822	-2.54372977669459\\
2.83041917808219	-2.58600325761041\\
2.84451643835616	-2.62799630357272\\
2.85861369863014	-2.66970988302638\\
2.87271095890411	-2.71114496441624\\
2.88680821917808	-2.75230251618715\\
2.90090547945205	-2.79318350678399\\
2.91500273972603	-2.83378890465159\\
2.9291	-2.87411967823482\\
2.94319726027397	-2.91417679597854\\
2.95729452054795	-2.95396122632759\\
2.97139178082192	-2.99347393772684\\
2.98548904109589	-3.03271589862114\\
2.99958630136986	-3.07168807745534\\
3.01368356164384	-3.11039144267431\\
3.02131714978317	-3.13123725158808\\
3.02778082191781	-3.1488269627229\\
3.04187808219178	-3.18699560604596\\
3.05597534246575	-3.22489834108835\\
3.07007260273973	-3.26253613629493\\
3.0841698630137	-3.29990996011055\\
3.09826712328767	-3.33702078098008\\
3.11236438356164	-3.37386956734835\\
3.12646164383562	-3.41045728766024\\
3.14055890410959	-3.4467849103606\\
3.15266757966406	-3.47778117988423\\
3.15465616438356	-3.48285340389427\\
3.16875342465753	-3.51866373670613\\
3.18285068493151	-3.55421687724102\\
3.19694794520548	-3.58951379394381\\
3.21104520547945	-3.62455545525933\\
3.22514246575342	-3.65934282963246\\
3.2392397260274	-3.69387688550806\\
3.25333698630137	-3.72815859133096\\
3.26743424657534	-3.76218891554604\\
3.28153150684932	-3.79596882659814\\
3.29562876712329	-3.82949929293213\\
3.30972602739726	-3.86278128299286\\
3.32382328767123	-3.89581576522518\\
3.33792054794521	-3.92860370807395\\
3.35201780821918	-3.96114607998403\\
3.35685684376248	-3.97226015701775\\
3.36611506849315	-3.99344384940028\\
3.38021232876712	-4.02549798476754\\
3.3943095890411	-4.05730945453067\\
3.40840684931507	-4.08887922713454\\
3.42250410958904	-4.120208271024\\
3.43660136986301	-4.1512975546439\\
3.45069863013699	-4.1821480464391\\
3.46479589041096	-4.21276071485445\\
3.47889315068493	-4.24313652833481\\
3.47983949243154	-4.24516718113695\\
3.4929904109589	-4.27327645532505\\
3.50708767123288	-4.30318146427\\
3.52118493150685	-4.33285252361453\\
3.53528219178082	-4.3622906018035\\
3.54937945205479	-4.39149666728176\\
3.56347671232877	-4.42047168849417\\
3.57757397260274	-4.44921663388557\\
3.59167123287671	-4.47773247190084\\
3.60576849315069	-4.50602017098483\\
3.61986575342466	-4.53408069958238\\
3.63396301369863	-4.56191502613837\\
3.6480602739726	-4.58952411909763\\
3.65525893764437	-4.6035359422315\\
3.66215753424658	-4.61690894690504\\
3.67625479452055	-4.64407047800544\\
3.69035205479452	-4.67100968084369\\
3.70444931506849	-4.69772752386465\\
3.71854657534247	-4.72422497551317\\
3.73264383561644	-4.75050300423411\\
3.74674109589041	-4.77656257847233\\
3.76083835616438	-4.80240466667268\\
3.77493561643836	-4.82803023728001\\
3.78903287671233	-4.85344025873919\\
3.8031301369863	-4.87863569949506\\
3.81722739726027	-4.90361752799249\\
3.83132465753425	-4.92838671267634\\
3.8368240849329	-4.93799187503242\\
3.84542191780822	-4.95294422199145\\
3.85951917808219	-4.97729102438268\\
3.87361643835616	-5.0014280882949\\
3.88771369863014	-5.02535638217295\\
3.90181095890411	-5.04907687446169\\
3.91590821917808	-5.07259053360598\\
3.93000547945205	-5.09589832805067\\
3.94410273972603	-5.11900122624062\\
3.9582	-5.14190019662068\\
3.97229726027397	-5.16459620763572\\
3.98639452054795	-5.18709022773058\\
4.00049178082192	-5.20938322535013\\
4.01458904109589	-5.23147616893922\\
4.02238399782767	-5.24360673091371\\
4.02868630136986	-5.2533700269427\\
4.04278356164384	-5.27506576780543\\
4.05688082191781	-5.29656435997227\\
4.07097808219178	-5.31786677188808\\
4.08507534246575	-5.3389739719977\\
4.09917260273973	-5.359886928746\\
4.1132698630137	-5.38060661057784\\
4.12736712328767	-5.40113398593805\\
4.14146438356164	-5.42147002327151\\
4.15556164383562	-5.44161569102307\\
4.16965890410959	-5.46157195763758\\
4.18375616438356	-5.48133979155992\\
4.19785342465753	-5.50092016123491\\
4.21195068493151	-5.52031403510743\\
4.22604794520548	-5.53952238162233\\
4.24014520547945	-5.55854616922446\\
4.25424246575342	-5.57738636635869\\
4.2683397260274	-5.59604394146986\\
4.28243698630137	-5.61451986300283\\
4.29349757932355	-5.6288893730329\\
4.29653424657534	-5.63281509940247\\
4.31063150684932	-5.65093061911362\\
4.32472876712329	-5.66886739058114\\
4.33882602739726	-5.68662638224989\\
4.35292328767123	-5.70420856256473\\
4.36702054794521	-5.7216148999705\\
4.38111780821918	-5.73884636291207\\
4.39521506849315	-5.75590391983429\\
4.40931232876712	-5.77278853918202\\
4.4234095890411	-5.78950118940011\\
4.42361181780061	-5.78973969015524\\
4.43750684931507	-5.80604283893342\\
4.45160410958904	-5.82241445622681\\
4.46570136986301	-5.83861700972512\\
4.47979863013699	-5.85465146787323\\
4.49389589041096	-5.87051879911598\\
4.50799315068493	-5.88621997189822\\
4.5220904109589	-5.90175595466483\\
4.53618767123288	-5.91712771586064\\
4.55028493150685	-5.93233622393053\\
4.56438219178082	-5.94738244731933\\
4.5784794520548	-5.96226735447192\\
4.59257671232877	-5.97699191383315\\
4.60667397260274	-5.99155709384786\\
4.62077123287671	-6.00596386296092\\
4.63407100519848	-6.01941128383268\\
4.63486849315069	-6.02021318961718\\
4.64896575342466	-6.03430604226151\\
4.66306301369863	-6.04824338933875\\
4.6771602739726	-6.06202619929376\\
4.69125753424658	-6.0756554405714\\
4.70535479452055	-6.08913208161653\\
4.71945205479452	-6.10245709087399\\
4.73354931506849	-6.11563143678865\\
4.74764657534247	-6.12865608780536\\
4.76174383561644	-6.14153201236898\\
4.77584109589041	-6.15426017892436\\
4.78993835616438	-6.16684155591636\\
4.80403561643836	-6.17927711178984\\
4.81813287671233	-6.19156781498964\\
4.8322301369863	-6.20371463396064\\
4.84632739726027	-6.21571853714768\\
4.86042465753425	-6.22758049299562\\
4.87136774785384	-6.23669117085117\\
4.87452191780822	-6.23930146994932\\
4.88861917808219	-6.25088243645363\\
4.90271643835616	-6.2623243609534\\
4.91681369863014	-6.2736282118935\\
4.93091095890411	-6.28479495771878\\
4.94500821917808	-6.29582556687409\\
4.95910547945206	-6.3067210078043\\
4.97320273972603	-6.31748224895426\\
4.9873	-6.32811025876882\\
4.99281381728739	-6.33223112292071\\
5.00139726027397	-6.33860600569283\\
5.01549452054795	-6.34897045817117\\
5.02959178082192	-6.35920458464867\\
5.04368904109589	-6.3693093535702\\
5.05778630136986	-6.37928573338062\\
5.07188356164384	-6.38913469252478\\
5.08598082191781	-6.39885719944753\\
5.10007808219178	-6.40845422259373\\
5.11417534246575	-6.41792673040824\\
5.12827260273973	-6.42727569133592\\
5.1423698630137	-6.43650207382162\\
5.15646712328767	-6.44560684631019\\
5.17056438356164	-6.4545909772465\\
5.18466164383562	-6.46345543507539\\
5.19434471374659	-6.46947538991085\\
5.19875890410959	-6.47220118824172\\
5.21285616438356	-6.48082920519036\\
5.22695342465753	-6.48934045436615\\
5.24105068493151	-6.49773590421396\\
5.25514794520548	-6.50601652317863\\
5.26924520547945	-6.51418327970502\\
5.28334246575342	-6.522237142238\\
5.2974397260274	-6.53017907922241\\
5.31153698630137	-6.53801005910311\\
5.32563424657534	-6.54573105032496\\
5.33973150684932	-6.55334302133282\\
5.35382876712329	-6.56084694057153\\
5.36792602739726	-6.56824377648596\\
5.37865808394189	-6.57380369576236\\
5.38202328767123	-6.57553449752097\\
5.39612054794521	-6.5827200721214\\
5.41021780821918	-6.58980146873211\\
5.42431506849315	-6.59677965579796\\
5.43841232876712	-6.60365560176382\\
5.4525095890411	-6.61043027507452\\
5.46660684931507	-6.61710464417493\\
5.48070410958904	-6.6236796775099\\
5.49480136986301	-6.6301563435243\\
5.50889863013699	-6.63653561066297\\
5.52299589041096	-6.64281844737078\\
5.53709315068493	-6.64900582209257\\
5.5511904109589	-6.6550987032732\\
5.56528767123288	-6.66109805935754\\
5.57938493150685	-6.66700485879043\\
5.59348219178082	-6.67282007001673\\
5.60757945205479	-6.6785446614813\\
5.62167671232877	-6.684179601629\\
5.63577397260274	-6.68972585890467\\
5.63740106851146	-6.69036033943632\\
5.64987123287671	-6.69518440175319\\
5.66396849315069	-6.70055619861939\\
5.67806575342466	-6.70584221794814\\
5.69216301369863	-6.7110434281843\\
5.7062602739726	-6.71616079777271\\
5.72035753424658	-6.72119529515825\\
5.73445479452055	-6.72614788878575\\
5.74855205479452	-6.73101954710008\\
5.76264931506849	-6.7358112385461\\
5.77674657534247	-6.74052393156866\\
5.79084383561644	-6.74515859461261\\
5.80494109589041	-6.74971619612282\\
5.81670232922919	-6.75346030229808\\
5.81903835616438	-6.75419770454413\\
5.83313561643836	-6.75860408832141\\
5.84723287671233	-6.7629363158995\\
5.8613301369863	-6.76719535572328\\
5.87542739726027	-6.77138217623758\\
5.88952465753425	-6.77549774588728\\
5.90362191780822	-6.77954303311721\\
5.91771917808219	-6.78351900637226\\
5.93181643835617	-6.78742663409725\\
5.94591369863014	-6.79126688473706\\
5.96001095890411	-6.79504072673653\\
5.97410821917808	-6.79874912854053\\
5.98820547945206	-6.80239305859391\\
6.00230273972603	-6.80597348534153\\
6.0164	-6.80949137722824\\
};
\end{axis}
\end{tikzpicture}%

==> Figs/Revise2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.07059,0.40784,0.70196}%
%
\begin{tikzpicture}

\begin{axis}[%
width=11.076in,
height=6.995in,
at={(1.858in,0.944in)},
scale only axis,
xmin=0,
xmax=6,
ymin=-7,
ymax=-4.5,
axis background/.style={fill=white}
]
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
0.856686385900919	-4.53532181968934\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
0.955945551252391	-4.73170715416063\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1.17426419331682	-5.02937618895169\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1.33960196941994	-5.30087076150997\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
1.69444274006365	-5.64490270652331\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
2.39177270923604	-6.05404448133452\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
3.29577661200145	-6.36628986988536\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
4.22119289042782	-6.65554931288377\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
4.57169193385716	-6.65247544741582\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
4.88442035440476	-6.71648869962701\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
5.26534782560261	-6.72186451848526\\
};
\addplot [color=blue, draw=none, mark size=5.0pt, mark=o, mark options={solid, blue}, forget plot]
  table[row sep=crcr]{%
5.95359933305229	-6.84645236272709\\
};
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
0.85	-4.61662524244643\\
0.856686385900919	-4.62592119352267\\
0.86763698630137	-4.6410802735534\\
0.88527397260274	-4.66532541681164\\
0.90291095890411	-4.68936166367799\\
0.920547945205479	-4.71319000560929\\
0.938184931506849	-4.73681143406241\\
0.955821917808219	-4.76022694049418\\
0.955945551252391	-4.76039035630068\\
0.973458904109589	-4.78343751636146\\
0.991095890410959	-4.80644415312111\\
1.00137724453597	-4.81976200620532\\
1.00873287671233	-4.82924784222996\\
1.0263698630137	-4.85184957514486\\
1.04400684931507	-4.87425034332268\\
1.06164383561644	-4.89645113822026\\
1.07928082191781	-4.91845295129444\\
1.09691780821918	-4.94025677400208\\
1.10526847157437	-4.95051154906045\\
1.11455479452055	-4.96186359780003\\
1.13219178082192	-4.98327441414513\\
1.14982876712329	-5.00449021449424\\
1.16746575342466	-5.02551199030421\\
1.17426419331682	-5.03356354917344\\
1.18510273972603	-5.04634073303188\\
1.2027397260274	-5.06697743413411\\
1.22037671232877	-5.08742308506775\\
1.23801369863014	-5.10767867728964\\
1.25565068493151	-5.12774520225664\\
1.27328767123288	-5.14762365142559\\
1.28284203440226	-5.15831407838751\\
1.29092465753425	-5.16731501625335\\
1.30856164383562	-5.18682028819677\\
1.32619863013699	-5.20614045871269\\
1.33960196941994	-5.22069976881568\\
1.34383561643836	-5.22527651925796\\
1.36147260273973	-5.24422946128944\\
1.3791095890411	-5.26300027626397\\
1.39674657534247	-5.28158995563841\\
1.40901924035567	-5.294419201286\\
1.41438356164384	-5.2999994908696\\
1.43202054794521	-5.31822987341439\\
1.44965753424658	-5.33628209472964\\
1.46729452054795	-5.35415714627219\\
1.48493150684932	-5.3718560194989\\
1.50256849315068	-5.38937970586661\\
1.52020547945205	-5.40672919683217\\
1.53784246575342	-5.42390548385243\\
1.55547945205479	-5.44090955838425\\
1.57311643835616	-5.45774241188446\\
1.57646553009519	-5.46091954483484\\
1.59075342465753	-5.47440503580993\\
1.6083904109589	-5.4908984216175\\
1.62602739726027	-5.50722356076403\\
1.64366438356164	-5.52338144470635\\
1.66130136986301	-5.53937306490132\\
1.67893835616438	-5.5551994128058\\
1.69444274006365	-5.56897637593432\\
1.69657534246575	-5.57086147987663\\
1.71421232876712	-5.58636025757066\\
1.73184931506849	-5.60169673734473\\
1.74948630136986	-5.61687191065571\\
1.76712328767123	-5.63188676896044\\
1.7847602739726	-5.64674230371577\\
1.79700955238106	-5.65696657369388\\
1.80239726027397	-5.66143950637854\\
1.82003424657534	-5.67597936840562\\
1.83767123287671	-5.69036288125385\\
1.85530821917808	-5.70459103638007\\
1.87294520547945	-5.71866482524115\\
1.89058219178082	-5.73258523929392\\
1.90821917808219	-5.74635326999524\\
1.92585616438356	-5.75996990880196\\
1.94349315068493	-5.77343614717092\\
1.9611301369863	-5.78675297655899\\
1.97876712328767	-5.799921388423\\
1.99640410958904	-5.81294237421981\\
2.01404109589041	-5.82581692540627\\
2.03167808219178	-5.83854603343922\\
2.04931506849315	-5.85113068977553\\
2.06510176064452	-5.86227338778356\\
2.06695205479452	-5.86357188587202\\
2.08458904109589	-5.87587061318557\\
2.10222602739726	-5.88802786317301\\
2.11986301369863	-5.90004462729119\\
2.1375	-5.91192189699697\\
2.15513698630137	-5.9236606637472\\
2.17277397260274	-5.93526191899872\\
2.19041095890411	-5.94672665420839\\
2.20047243051213	-5.95320623187961\\
2.20804794520548	-5.95805586083306\\
2.22568493150685	-5.96925053032957\\
2.24332191780822	-5.98031165415477\\
2.26095890410959	-5.99124022376552\\
2.27859589041096	-6.00203723061866\\
2.29623287671233	-6.01270366617104\\
2.3138698630137	-6.02324052187952\\
2.33150684931507	-6.03364878920095\\
2.34914383561644	-6.04392945959216\\
2.36678082191781	-6.05408352451002\\
2.38441780821918	-6.06411197541138\\
2.39177270923604	-6.06825711958017\\
2.40205479452055	-6.07401580375307\\
2.41969178082192	-6.08379600099196\\
2.43732876712329	-6.09345355858489\\
2.45496575342466	-6.10298946798871\\
2.47260273972603	-6.11240472066028\\
2.4902397260274	-6.12170030805644\\
2.50787671232877	-6.13087722163404\\
2.52551369863014	-6.13993645284993\\
2.54315068493151	-6.14887899316096\\
2.56078767123288	-6.15770583402398\\
2.57842465753425	-6.16641796689584\\
2.59606164383562	-6.1750163832334\\
2.59739594105384	-6.17566228326089\\
2.61369863013699	-6.18350207449349\\
2.63133561643836	-6.19187603213298\\
2.64897260273973	-6.2001392476087\\
2.6666095890411	-6.20829271237752\\
2.68424657534247	-6.21633741789627\\
2.70188356164384	-6.22427435562182\\
2.71952054794521	-6.232104517011\\
2.73715753424658	-6.23982889352067\\
2.75479452054795	-6.24744847660768\\
2.77243150684932	-6.25496425772888\\
2.79006849315068	-6.26237722834112\\
2.80770547945206	-6.26968837990125\\
2.82534246575342	-6.27689870386612\\
2.84297945205479	-6.28400919169257\\
2.86061643835616	-6.29102083483746\\
2.87825342465753	-6.29793462475764\\
2.8958904109589	-6.30475155290995\\
2.91352739726027	-6.31147261075126\\
2.93116438356164	-6.3180987897384\\
2.93133883546455	-6.3181638603955\\
2.94880136986301	-6.32463108132822\\
2.96643835616438	-6.33107047697759\\
2.98407534246575	-6.33741796814334\\
3.00171232876712	-6.34367454628232\\
3.01934931506849	-6.34984120285139\\
3.03698630136986	-6.3559189293074\\
3.05462328767123	-6.36190871710719\\
3.0722602739726	-6.36781155770762\\
3.08989726027397	-6.37362844256554\\
3.10753424657534	-6.37936036313778\\
3.12517123287671	-6.38500831088122\\
3.14280821917808	-6.39057327725268\\
3.16044520547945	-6.39605625370904\\
3.17808219178082	-6.40145823170712\\
3.19571917808219	-6.40678020270379\\
3.21335616438356	-6.4120231581559\\
3.23099315068493	-6.41718808952029\\
3.2486301369863	-6.42227598825381\\
3.26626712328767	-6.42728784581331\\
3.28390410958904	-6.43222465365565\\
3.29577661200145	-6.43550614521811\\
3.30154109589041	-6.43708740323767\\
3.31917808219178	-6.44187708601622\\
3.33681506849315	-6.44659469344815\\
3.35445205479452	-6.45124121699032\\
3.37208904109589	-6.45581764809957\\
3.38972602739726	-6.46032497823275\\
3.40736301369863	-6.46476419884671\\
3.425	-6.46913630139831\\
3.44263698630137	-6.47344227734438\\
3.46027397260274	-6.47768311814179\\
3.47791095890411	-6.48185981524738\\
3.49554794520548	-6.48597336011799\\
3.51318493150685	-6.49002474421049\\
3.53082191780822	-6.49401495898172\\
3.54845890410959	-6.49794499588853\\
3.56609589041096	-6.50181584638776\\
3.58373287671233	-6.50562850193628\\
3.6013698630137	-6.50938395399093\\
3.61900684931507	-6.51308319400856\\
3.63664383561644	-6.51672721344601\\
3.65428082191781	-6.52031700376014\\
3.67191780821918	-6.52385355640781\\
3.68955479452055	-6.52733786284585\\
3.70719178082192	-6.53077091453112\\
3.72482876712329	-6.53415370292046\\
3.74246575342466	-6.53748721947074\\
3.75861177589174	-6.54049657796109\\
3.76010273972603	-6.54077245563879\\
3.7777397260274	-6.54401040288147\\
3.79537671232877	-6.54720205265563\\
3.81301369863014	-6.55034839641812\\
3.83065068493151	-6.55345042562578\\
3.84828767123288	-6.55650913173547\\
3.86592465753425	-6.55952550620403\\
3.88356164383562	-6.56250054048832\\
3.90119863013699	-6.56543522604519\\
3.91883561643836	-6.56833055433148\\
3.93647260273973	-6.57118751680405\\
3.9541095890411	-6.57400710491974\\
3.97174657534247	-6.57679031013541\\
3.98938356164384	-6.57953812390791\\
4.00702054794521	-6.58225153769408\\
4.02465753424658	-6.58493154295077\\
4.04229452054795	-6.58757913113484\\
4.05993150684932	-6.59019529370313\\
4.07756849315069	-6.5927810221125\\
4.09520547945205	-6.59533730781979\\
4.11284246575342	-6.59786514228185\\
4.13047945205479	-6.60036551695554\\
4.14811643835616	-6.6028394232977\\
4.16575342465753	-6.60528785276518\\
4.1833904109589	-6.60771179681484\\
4.20102739726027	-6.61011224690352\\
4.21866438356164	-6.61249019448807\\
4.22119289042782	-6.61282932007375\\
4.23630136986301	-6.61484663102535\\
4.25393835616438	-6.61718254797219\\
4.27157534246575	-6.61949893678546\\
4.28921232876712	-6.621796788922\\
4.30684931506849	-6.62407709583867\\
4.32448630136986	-6.6263408489923\\
4.34212328767123	-6.62858903983975\\
4.3597602739726	-6.63082265983788\\
4.37739726027397	-6.63304270044352\\
4.39503424657534	-6.63525015311354\\
4.41267123287671	-6.63744600930478\\
4.43030821917808	-6.63963126047408\\
4.44794520547945	-6.64180689807831\\
4.46558219178082	-6.64397391357431\\
4.48321917808219	-6.64613329841892\\
4.50085616438356	-6.64828604406901\\
4.51849315068493	-6.65043314198141\\
4.5361301369863	-6.65257558361299\\
4.55376712328767	-6.65471436042058\\
4.57140410958904	-6.65685046386104\\
4.57169193385716	-6.65688530705099\\
4.58904109589041	-6.65898488539122\\
4.60667808219178	-6.66111861646797\\
4.62431506849315	-6.66325264854813\\
4.64195205479452	-6.66538797308856\\
4.65958904109589	-6.66752558154611\\
4.67722602739726	-6.66966646537763\\
4.69486301369863	-6.67181161603997\\
4.7125	-6.67396202498997\\
4.73013698630137	-6.67611868368449\\
4.74777397260274	-6.67828258358037\\
4.76541095890411	-6.68045471613448\\
4.78304794520548	-6.68263607280364\\
4.80068493150685	-6.68482764504473\\
4.81832191780822	-6.68703042431458\\
4.83595890410959	-6.68924540207004\\
4.85359589041096	-6.69147356976797\\
4.87123287671233	-6.69371591886522\\
4.88442035440476	-6.69540242126539\\
4.8888698630137	-6.69597344081863\\
4.90650684931507	-6.69824712708505\\
4.92414383561644	-6.70053796912135\\
4.94178082191781	-6.70284695838435\\
4.95941780821918	-6.70517508633092\\
4.97705479452055	-6.7075233444179\\
4.99469178082192	-6.70989272410215\\
5.01232876712329	-6.71228421684051\\
5.02996575342466	-6.71469881408983\\
5.04760273972603	-6.71713750730697\\
5.0652397260274	-6.71960128794877\\
5.08287671232877	-6.72209114747208\\
5.10051369863014	-6.72460807733376\\
5.11815068493151	-6.72715306899065\\
5.13578767123288	-6.7297271138996\\
5.14334707003083	-6.73083951740014\\
5.15342465753425	-6.73233120351746\\
5.17106164383562	-6.73496632930108\\
5.18869863013699	-6.73763348270732\\
5.20633561643836	-6.74033365519301\\
5.22397260273973	-6.74306783821502\\
5.2416095890411	-6.74583702323019\\
5.25924657534247	-6.74864220169537\\
5.26534782560261	-6.74962117088711\\
5.27688356164384	-6.75148436506741\\
5.29452054794521	-6.75436450480316\\
5.31215753424658	-6.75728361235947\\
5.32979452054794	-6.7602426791932\\
5.34743150684931	-6.76324269676118\\
5.36506849315068	-6.76628465652027\\
5.38270547945206	-6.76936954992732\\
5.40034246575342	-6.77249836843918\\
5.41797945205479	-6.7756721035127\\
5.42731754097933	-6.77737099605476\\
5.43561643835616	-6.77889174660472\\
5.45325342465753	-6.78215828917211\\
5.4708904109589	-6.78547272267171\\
5.48852739726027	-6.78883603856036\\
5.50616438356164	-6.79224922829492\\
5.52380136986301	-6.79571328333224\\
5.54143835616438	-6.79922919512916\\
5.55907534246575	-6.80279795514255\\
5.57671232876712	-6.80642055482924\\
5.57965585775113	-6.80703046180824\\
5.59434931506849	-6.81009798564609\\
5.61198630136986	-6.81383123904994\\
5.62962328767123	-6.81762130649766\\
5.6472602739726	-6.82146917944608\\
5.66489726027397	-6.82537584935205\\
5.68253424657534	-6.82934230767243\\
5.70017123287671	-6.83336954586407\\
5.71780821917808	-6.83745855538381\\
5.73544520547945	-6.84161032768851\\
5.75308219178082	-6.84582585423501\\
5.77071917808219	-6.85010612648017\\
5.78835616438356	-6.85445213588083\\
5.80599315068493	-6.85886487389385\\
5.8110436127388	-6.86014091831871\\
5.8236301369863	-6.86334533197607\\
5.84126712328767	-6.86789450158435\\
5.85890410958904	-6.87251337417553\\
5.87654109589041	-6.87720294120647\\
5.89417808219178	-6.88196419413401\\
5.91181506849315	-6.886798124415\\
5.92945205479452	-6.89170572350629\\
5.94708904109589	-6.89668798286474\\
5.95359933305229	-6.89854613430779\\
5.96472602739726	-6.90174589394719\\
5.98236301369863	-6.9068804482105\\
6	-6.91209263711151\\
};
\end{axis}
\end{tikzpicture}%
